Evolutionary Hierarchical Harvest Schedule Optimization for Food Waste Prevention

In order to avoid disadvantages of monocropping for soil and environment, it is advisable to practice intercropping of various plant species whenever possible. However, intercropping is challenging as it requires a balanced planting schedule due to individual cultivation time frames. Maintaining a continuous harvest reduces logistical costs and related greenhouse gas emissions, and contributes to food waste prevention. In this work, we address these issues and propose an optimization method for a full harvest season of large crop ensembles that complies with given constraints. By using an approach based on an evolutionary algorithm combined with a novel hierarchical loss function and adaptive mutation rate, we transfer the multi-objective into a pseudo-single-objective optimization problem and obtain faster convergence and better solutions than for conventional approaches.

==> acknowledgement.tex <==
\section*{Acknowledgement}

This work was partially funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under Germany’s Excellence Strategy – EXC 2070 – 390732324.
Other parts were funded by the Federal Ministry of Education and Research of Germany as part of the competence center for machine learning ML2R (01IS18038B).

==> biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/maurice_guender.jpg}}]{Maurice Günder} recieved a B.Sc. degree in physics and a M.Sc. degree in experimental particle physics at RWTH Aachen University. Since 2020, he is a data scientist at Fraunhofer IAIS in Sankt Augustin, Germany, and a PhD candidate at the University of Bonn, Germany, with the Cluster of Excellence “PhenoRob”. His research interests comprise time series and image analysis, knowledge extraction from sensorial data, and process knowledge aided modelling.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/nico_piatkowski.png}}]{Dr. Nico Piatkowski} received his B.Sc., Dipl.-Inf. and Dr. rer. nat. degrees from TU Dortmund University, Dortmund, Germany. He is currently a senior research scientist at the Media Engineering Group of the Fraunhofer Institute for Intelligent Analysis and Information Systems IAIS in Sankt Augustin, Germany. Before that, he was a research scientist at the Artificial Intelligence Unit at TU Dortmund, at the DFG Collaborative Research Center SFB 876 on “Providing Information by Resource Constrained Data Analysis”, and then the Competence Center Machine Learning Rhine-Ruhr (ML2R). Nico contributed to various large-scale research projects on the foundations of machine learning under resource constraints, spatio-temporal modelling, and probabilistic inference. His current research is focused on quantum computing methods for structural and probabilistic inference. He is coordinator of the Quantum Machine Learning group at the competence center Machine Learning Rhine-Ruhr, funded by the Federal Ministry of Education and Research (BMBF) as one of six nationwide nodes for AI and ML research and transfer in Germany.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/laura_von_rueden.jpg}}]{Laura von Rueden} received a B.Sc. degree in physics and a M.Sc. degree in simulation sciences in 2015 from RWTH Aachen University. Afterwards, she was a data scientist at Capgemini. Since 2018, she is a research scientist at Fraunhofer IAIS and a PhD candidate in computer science at the Universität Bonn. Her research interests include machine learning and especially the combination of data- and knowledge-based modelling.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/rafet_sifa.jpg}}]{Dr. Rafet Sifa} is the deputy head of the Media Engineering Department, head of the business unit Cognitive Business Optimization and a senior research data scientist at Fraunhofer Institute for Intelligent Analysis and Information Systems (IAIS) in Sankt Augustin Germany. He is also currently teaching M.Sc. level data science courses as a guest lecturer to students of University of Bonn and RWTH Aachen University at the Bonn-Aachen International Center for Information Technology.

Rafet Sifa holds his Master's and PhD degrees in Computer Science from the University of Bonn in Germany. His current research focus is based on statistical data mining in the context of representation learning for a variety of industry applications involving behavioral analytics, medical informatics, accounting, digital forensics and text mining. Before joining Fraunhofer, he worked as a data scientist in the games industry, where he mainly concentrated on developing large scale machine learning solutions for business intelligence problems. He often gives talks and organizes workshops about representation learning and behavioral analytics in scientific conferences and industrial summits.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/christian_bauckhage.jpg}}]{Prof. Dr. Christian Bauckhage} (M’02) received his M.Sc. and Ph.D. degrees in computer science from Bielefeld University in 1998 and 2002, respectively. Since 2008, he is a professor of computer science at the University of Bonn and lead scientist for machine learning at Fraunhofer IAIS. Previously, he was with the Centre for Vision Research in Toronto, Canada and a Senior Research Scientist at Deutsche Telekom Laboratories, Berlin. His research focuses on theory and practice of learning systems and next generation computing. He regularly reviews for the IEEE Transactions on Neural Networks and Learning Systems, the IEEE Transactions on Pattern Analysis and Machine Intelligence, and the IEEE Transactions on Games for which he is also an associate editor.
\end{IEEEbiography}

